A non-parametric mixture model for topic modeling over time

A single, stationary topic model such as latent Dirichlet allocation is inappropriate for modeling corpora that span long time periods, as the popularity of topics is likely to change over time. A number of models that incorporate time have been proposed, but in general they either exhibit limited forms of temporal variation, or require computationally expensive inference methods. In this paper we propose non-parametric Topics over Time (npTOT), a model for time-varying topics that allows an unbounded number of topics and exible distribution over the temporal variations in those topics' popularity. We develop a collapsed Gibbs sampler for the proposed model and compare against existing models on synthetic and real document sets.

==> Results.tex <==
\section{Results}
\label{sec:results}
\subsubsection{State of the Union Address Dataset} The State-of-the-Union dataset \footnote{Downloaded from: {http://www.gutenberg.org/dirs/etext04/suall11.txt}} contains the transcripts of 208 State-of-the-Union addresses during 1790 to 2002. We followed \cite{wang:06} in processing the dataset. Namely, we divide each speech into three-paragraph documents, we remove stop words and numbers and we normalize the timestamps to the range $(0,1)$. Due to time constraints we run on a subset of the dataset covering the range of 1790 to 1814. In this experiment, we changed the sampling order to randomly go through words in different documents rather than sequentially processing each document. The reason behind this change is that we noticed that the model tends to fit a topic with a single time component of very high precision at each distinct timestamp. We attributed this to fact that the posterior distribution of time given multiple observations having the same timestamp will concentrate around this timestamp, which makes the model very likely to create a new time component when a new document with a different timestamp arrives. This problem did not occur in twitter data because each document contains only few words (maximum 18).

\subsection{Hyperparameter setting}
Setting the hyper-parameter to appropriate value is very important for good performance. We ran a dummy experiment to examine how the posterior distirbution over time changes when two points ($0.0$, $0.1$) are observed assuming that the time distirbution is normal with normal-gamma prior on the parameters. The result is shown in figure \ref{fig:prior}. Figure \ref{fig:prior}(a) shows that the posterior has higher probability than the prior even at places like $0.7$ and $0.8$ where there has been no observed points. This results from the skewness in the prior. Figure \ref{fig:prior} (b) shows that the posterior behaves as expected when the prior is flat. Therefore, we used a flat prior over time component parameters for all our experiments.
%
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth,height=0.2\textheight]{PriorAnalysis}
\caption{Both figures show how the posterior of normal-gamma distribution change when two points ($0.0$, and $0.1$) are seen from the same distribution}
\label{fig:prior}
\end{figure*}
%
\subsection{Synthetic Dataset}
First we present the result on the synthetic data set. On the synthetic data we ran TOT and npTOT. The number of topics in TOT was set to the true number of topics. A sample topic is shown in figure \ref{fig:Synthetic}.  We found that we were able to recover most of the topics using npTOT (npTOT detected 4 topics). While TOT was also able to discover topics, it was unable to accurately fit their multi-modal behavior with respect to time. 
\begin{figure}
\centering
\includegraphics[scale = .4]{Synthetic_V}
\caption{(a) shows the actual distribution over time for a particular topic on the synthetic data set, (b) shows the distribution over words for that particular topic, (c) shows the distribution over time of the TOT-detected topic closest to the original (d) shows the probability of the top-10 words for the TOT topics in (c), (e) shows the distribution over time for corresponding topic found by npTOT and (f) shows the word distribution for the npTOT topic in (e)}
\label{fig:Synthetic}
\end{figure}
%
\subsection{Real dataset results}
On real data sets, our model was able to capture topics with multiple time components (examples are shown in figure \ref{fig:real_data_stats} ). For example, in the State of the union dataset, it extracted a topic covering the US-Britain conflict that has multiple components corresponding to tensions leading to the war and the declaration of the war in 1812. On Twitter dataset, it fitted to components to model a fast growth but slow decline of interest in revolution in Libya. However, we observed that TOT is able to extract more meaningful topics. We believe that the performance of our model can be enhanced by using Gibbs sampling instead of SMC. Gibbs sampling revisits assigned latent variables (topics and time components) multiple times, resulting in a more reliable estimation. 
%
\begin{figure*}
\centering
\includegraphics[width=1.0\textwidth,height=0.3\textheight]{real_data_stats.png}
\caption{Sample topics extracted by npTOT model and corresponding TOT topics. For each topic, most probable 10 words are shown. \textbf{Left:} Libyan revolution in Twitter dataset. \textbf{Right:} US-Britain conflict in state of the union address dataset.}
\label{fig:real_data_stats}
\end{figure*}


==> introduction.tex <==
\section{Introduction}
With the exploding amount of document collections available in various domains, automatic extraction of abstractions of document collections has gained increasing interest. One particularly interesting form of abstraction is topic models. Topic models have evolved from mixture of unigram models, where each document is assigned to a single topic to models such as probabilistic Latent Semantic Indexing and Latent Dirichlet Allocation (LDA) \cite{blei:03}, where each document is assumed to be generated by a mixture of topics.

These models assume that our data is exchangeable -- i.e. that the order of our documents is not important, and that conditioned on a latent set of topics (multinomial distributions over words) and topic proportions (multinomial distributions over topics), the documents are i.i.d. Such a model cannot capture temporal variations (such as changes in topic composition or popularity over time), due to the exchangeability assumption. The multinomial distributions mean that they also cannot capture correlations between topics. A number of models have been developed to address these shortcomings. The Topics over Time (TOT) model \cite{wang:06} is an example of a model that takes into consideration temporal information by jointly modeling document words and timestamps. The Correlated Topic Model [cite] is an extension to LDA that incorporates correlations between topics; unfortunately, this model does not have the desirable conjugacy properties of LDA.

Another important advancement in topic modeling is the employment of nonparametric models, such as the Hierarchical Dirichlet Process [cite]. Nonparametric models allow the number of topics to grow with the documents rather than predetermining a fixed number of topics. 

In this work, we develop a nonparametric extension of TOT topic model that we call nonparametric Topics over Time (npTOT).
This model uses infinite dimensional mixtures  to model both word distribution and time distribution of each topic.
It is thus nonparametric with respect to the number of topics and also nonparametric with respect to distribution over time for each topic. This means that each of an unbounded number of topics can vary in popularity across time, with minimal restrictions on the form of this temporal variation. This is in contrast to the parametric TOT model, where each topic can only rise and fall in popularity once. As we see in figure~\ref{fig:multimodal}, real-world data does not exhibit such simple behavior. By coupling the distributions over time using a hierarchical Dirichlet process, npTOT can induce correlations between topics, without needing to resort to non-conjugate distributions.


%The later aspect gives the model enough flexibility to model topics with multimodel distributions over times, which do occur in real-word data (See figure \ref{fig:multimodal}).

\begin{figure}
\label{fig:multimodal}
\includegraphics[width=0.45\textwidth,height=0.25\textheight]{multimodal.png}
\caption{Search and news trends for "NHL" obtained from Google Trends. This shows that interest in this topic (as well as its content in the news) does rise and fall multiple times.}
\end{figure}

We compare the performance of our model with that of Topics over Time (TOT) \cite{wang:06}, which uses parametric models for word and time distributions and does not couple the distributions over time.

The rest of the paper is organized as follows: In section \ref{sec:related}, we review related literature on topic modeling, including the base-line TOT model. In section \ref{sec:nptot} we describe our proposed npTOT model. Section \ref{sec:inference} describes the inference scheme. Experimental setup and results are described in section \ref{sec:exp}, and finally we conclude in \ref{sec:conclusions}.

